Coordinate-space calculation of the window observable for the hadronic vacuum polarization contribution to $(g-2)_\mu$

The `intermediate window quantity' of the hadronic vacuum polarization contribution to the anomalous magnetic moment of the muon allows for a high-precision comparison between the data-driven approach and lattice QCD. The existing lattice results, which presently show good consistency among each other, are in strong tension with the data-driven determination. In order to check for a potentially common source of systematic error of the lattice calculations, which are all based on the time-momentum representation (TMR), we perform a calculation using a Lorentz-covariant coordinate-space (CCS) representation. We present results for the isovector and the connected strange-quark contributions to the intermediate window quantity at a reference point in the $(m_\pi,m_K)$ plane, in the continuum and infinite-volume limit, based on four different lattice spacings. Our results are in good agreement with those of the recent TMR-based Mainz-CLS publication.

==> ccs_integrand.tex <==
\subsection{CCS integrand for the different kernels}
As mentioned in section \ref{section:ccs_method} the calculation in the CCS method leaves the freedom of choosing among a family of kernel functions. This choice does not affect the infinite volume result. But, the shape of the integrand can be very different for a different kernel functions. A comparison of the integrand is shown in figure \ref{fig:ccs_integrand}. It is desirable to choose a more short-ranged kernel, to reach convergence of the integrand at a shorter distance than the lattice size. However, more short-ranged kernels, i.e. $H^{\textrm{XX}}_{\mu\nu}(x)$, show a subtle oscillatory behaviour, when approaching zero, which can affect the results, especially for smaller ensembles. This means, that it is crucial for these ensembles to choose a well suited kernel functions.\\
On the other hand, this observation can be used to justify the stability of the results for a given ensemble. If several different kernel functions agree on the final result, the convergence of the data in the box is very good.\\
For the window quantity we do not perform any additional treatment of the tail of the integrand.

\begin{figure}
\begin{subfigure}{0.49\textwidth}
     \centering
    \includegraphics[width=0.9\textwidth]{ccs_integrand_N203.pdf}
    \caption{N203 (L=3.1fm)}
    \label{fig:my_label}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
     \centering
    \includegraphics[width=0.9\textwidth]{ccs_integrand_N302.pdf}
    \caption{N302 (L=2.4fm)}
    \label{fig:my_label}
\end{subfigure}
\caption{Comparison of the integrand for different kernels on two different ensembles \julian{redo the plots}}
\label{fig:ccs_integrand}
\end{figure}
